Deep Rigid Instance Scene Flow

In this paper we tackle the problem of scene flow estimation in the context of self-driving. We leverage deep learning techniques as well as strong priors as in our application domain the motion of the scene can be composed by the motion of the robot and the 3D motion of the actors in the scene. We formulate the problem as energy minimization in a deep structured model, which can be solved efficiently in the GPU by unrolling a Gaussian-Newton solver. Our experiments in the challenging KITTI scene flow dataset show that we outperform the state-of-the-art by a very large margin, while being 800 times faster.

==> dataset.tex <==
%!TEX root = top.tex
\section{Curating KITTI Scene Flow}
In order to evaluate the 3D rigid motion estimates produced by our system, we must have enough labeled data.
However, to our knowledge, no dataset has such
Fortunately, KITTI Scene flow dataset provides ground truth for optical flow, disparity, and instance segmentation. We can use the data to fit a rigid motion for each object instance.

We discover two critical issues: first, there are mis-alignments between GT flow/disparity and GT segmentation. Second, the scale of the same 3D CAD model sometimes change across frames.

The first issue is due to the fact that the GT are collected via different means. While the GT flow and GT disparity are obtained from the fitted 3D CAD model, the GT segmentation are based on human annotation. For instance, we can often observe that the side mirrors of the vehicles are ignored by the annotator. When using the GT obtained by CAD model for evaluation, the error will accumulate and hurt the performance.

We first use the GT segmentation mask to define each object instance. Then we fit a rigid motion using the GT flow and GT disparity of each instance with least square objective. Since some pixels may be mis-labeled by the annotators, for each pixel we search if there are other instances in the surrounding area, and if there are, we transform the pixel with their rigid motion. If their rigid motion better explains the pixel's 3D movement, \emph{i.e.} the 3D distance are closer, then we assign the pixel to that instance. At the end, we perform the SVD fitting again with the new pixel assignment.

Even after re-labeling, there are still a few vehicle instances where our rigid motion cannot explain very well. After careful diagnose, we notice that this is because the scale of the CAD model changes across frames. To verify our hypothesis, we compute the eigen decomposition for the same instance across frames. Ideally if the scale of the instance does not change much, the eigen value should be roughly the same. Unfortunately, we discover a few examples where the largest eigen value changes by $7\%$. We also tried to measure the 3D distance between two points in consecutive frames. The distance in theory shall remain fixed due to rigid motion. Yet it changed as well.

==> table_energy_ablation.tex <==
\begin{table*}[tb]
\centering
\begin{tabular}{ccccccc}
\specialrule{.2em}{.1em}{.1em}
%\hline
\multicolumn{3}{c}{Employed energy}&\multicolumn{4}{c}{Background outliers (\%)}\\
${E}_{pho}$& ${E}_{flow}$&${E}_{rigid}$ &D1&{D2} &{Fl}  &{SF}\\
\hline
\checkmark& & &1.92 &2.69 &{\bf3.71} &{\bf4.30}  \\
%& \checkmark&  &1.92 & 2.57 &4.73 &5.31\\
%&& \checkmark &1.92 &2.59 & 5.92 &6.45\\
\checkmark& \checkmark& &1.92 & 2.57 & 4.25 & 4.82\\
& \checkmark& \checkmark &1.92 & 2.56& 4.72& 5.28\\
\checkmark& &\checkmark &1.92 &{\bf2.55} &4.69 &5.25\\
\checkmark& \checkmark & \checkmark &1.92 &2.56 &4.63 &5.21\\
\specialrule{.1em}{.05em}{.05em}
\end{tabular}
\begin{tabular}{ccccccc}
\specialrule{.2em}{.1em}{.1em}
%\hline
\multicolumn{3}{c}{Employed energy}&\multicolumn{4}{c}{Foreground outliers (\%)}\\
${E}_{pho}$& ${E}_{flow}$&${E}_{rigid}$ &D1&{D2} &{Fl}  &{SF}\\
\hline
\checkmark& & &1.70 &4.25 &7.57 &9.00 \\
& \checkmark&  &1.70& 5.53 &8.39 &10.5\\
&& \checkmark  &1.70 &3.72 &14.9 &16.1\\
\checkmark& \checkmark&  &1.70 & 5.18 & 7.97 & 9.85\\
& \checkmark& \checkmark &1.70 & 4.58 & 6.98 & 8.67\\
\checkmark& &\checkmark &1.70 &{\bf3.70} &7.98 &9.24\\
\checkmark& \checkmark & \checkmark &1.70 &4.56 &{\bf6.73} &{\bf8.39}\\
\specialrule{.1em}{.05em}{.05em}
\end{tabular}
\caption{\textbf{Contributions of each energy:}}
\label{tab:ablation-energy}
\end{table*}
